Searches for the Higgs boson at the LHC

The search strategy for the Standard Model Higgs boson at the Large Hadron Collider is reviewed, with a particular emphasis on its potential observation by the ATLAS and CMS detectors in the $\gamma\gamma$, $\tau^+\tau^-$, $ZZ^{*}$ and $WW^{*}$ final states. The combined Higgs discovery potential of ATLAS and CMS is discussed, as well as the expected exclusion limits on the production rate times the branching ratio as a function of the Higgs mass and the collected luminosity.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = delmastro-blois-2009

default: pdf

note:
	latex  ${BASENAME}
	latex  ${BASENAME}
	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}

pdf: note	
	rm -f    ${BASENAME}.ps.gz
	dvips -o ${BASENAME}.ps ${BASENAME}
	ps2pdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}.ps ${BASENAME}.pdf
	gzip -f  ${BASENAME}.ps

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp *.ps* *.pdf


